On Formal Methods for Collective Adaptive System Engineering. {Scalable Approximated, Spatial} Analysis Techniques. Extended Abstract

In this extended abstract a view on the role of Formal Methods in System Engineering is briefly presented. Then two examples of useful analysis techniques based on solid mathematical theories are discussed as well as the software tools which have been built for supporting such techniques. The first technique is Scalable Approximated Population DTMC Model-checking. The second one is Spatial Model-checking for Closure Spaces. Both techniques have been developed in the context of the EU funded project QUANTICOL.

==> eptcsdata.tex <==
\providecommand{\firstpage}{53}
\providecommand{\publicationstatus}{M.H. ter Beek and M. Loreti (Eds.): Workshop on\\ 
FORmal methods for the quantitative Evaluation\\ 
of Collective Adaptive SysTems (FORECAST'16).\\
EPTCS 217, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.217.7}{10.4204/EPTCS.217.7}}

